Enhancing Performance on Seen and Unseen Dialogue Scenarios using Retrieval-Augmented End-to-End Task-Oriented System

End-to-end task-oriented dialogue (TOD) systems have achieved promising performance by leveraging sophisticated natural language understanding and natural language generation capabilities of pre-trained models. This work enables the TOD systems with more flexibility through a simple cache. The cache provides the flexibility to dynamically update the TOD systems and handle both existing and unseen dialogue scenarios. Towards this end, we first fine-tune a retrieval module to effectively retrieve the most relevant information entries from the cache. We then train end-to-end TOD models that can refer to and ground on both dialogue history and retrieved information during TOD generation. The cache is straightforward to construct, and the backbone models of TOD systems are compatible with existing pre-trained generative models. Extensive experiments demonstrate the superior performance of our framework, with a notable improvement in non-empty joint goal accuracy by 6.7% compared to strong baselines.

==> exp_results_copy.tex <==

% \begin{table*}[]
% \centering
% \resizebox{0.98\linewidth}{!}{
% \begin{tabular}{l|ccccccc}
% \hline
%                                                                                                                                           & PPL   & JGA    & Empty JGA & Non-Empty JGA & Token ACC & Token EM & BLEU-4 \\ \hline
% BART-Large                                                                                                                                & 1.700 & 0.8760 & 0.9918    & 0.5864        & 0.8754    & 0.5379   & 0.2205 \\ \hline
% INTENT: intent name, SLOT: slot name                                                                                                      & 1.688 & 0.8891 & 0.9914    & 0.6329        & 0.8710    & 0.5384   & 0.2121 \\ \hdashline
% intent name, slot name, intent description, slot description                                                                              & 1.679 & 0.8947 & 0.9881    & 0.6610        & 0.8716    & 0.5409   & 0.2145 \\ \hdashline
% \begin{tabular}[c]{@{}l@{}}intent name, slot name, service description,\\ intent description, slot description\end{tabular}               & 1.679 & 0.8939 & 0.9918    & 0.6490        & 0.8713    & 0.5409   & 0.2116 \\ \hdashline
% \begin{tabular}[c]{@{}l@{}}INTENT: intent name, service description,\\ intent description, SLOT: slot name, slot description\end{tabular} & 1.676 & 0.8968 & 0.9913    & 0.6604        & 0.8726    & 0.5440   & 0.2172 \\ \hline
% \end{tabular}}\caption{Performance of FiD-TOD with variants of cache on the development set.  }\label{table:variants-of-db}
% \vspace{-0.5em}
% \end{table*}

\begin{table*}[]
\centering
\resizebox{0.98\linewidth}{!}{
\begin{tabular}{l|cccccc}
\hline
                                                                                                                                          & PPL   & JGA    &  Unseen JGA & Token ACC & Token EM & BLEU-4 \\ \hline
BART-Large                                                                                                                                & 1.700 & 0.876     & 0.586        & \textbf{0.875}    & 0.538   & \textbf{0.221} \\ \hline
INTENT: intent name, SLOT: slot name                                                                                                      & 1.688 & 0.889    & 0.633        & 0.871    & 0.538   & 0.212 \\ \hdashline
intent name, slot name, intent description, slot description                                                                              & 1.679 & 0.895    & \textbf{0.661}        & 0.872    & 0.541   & 0.215 \\ \hdashline
\begin{tabular}[c]{@{}l@{}}intent name, slot name, service description,\\ intent description, slot description\end{tabular}               & 1.679 & 0.894     & 0.649        & 0.871    & 0.541   & 0.212 \\ \hdashline
\begin{tabular}[c]{@{}l@{}}INTENT: intent name, service description,\\ intent description, SLOT: slot name, slot description\end{tabular} & \textbf{1.676} & \textbf{0.897}     & 0.660        & 0.873    & \textbf{0.545}   & 0.217 \\ \hline
\end{tabular}}\caption{Performance of FiD-TOD with variants of cache on the development set.  }\label{table:variants-of-db}
 \vspace{-0.5em}
\end{table*}
%%%%%%%%%%%%%

% \begin{table*}[]
% \centering
% \resizebox{0.98\linewidth}{!}{
% \begin{tabular}{l|ccccccc}
% \hline
%                                  & PPL   & JGA    & Empty JGA & Non-Empty JGA & Token ACC & Token EM & BLEU-4 \\ \hline
% BART-Large                       & 1.700 & 0.8760 & 0.9918    & 0.5864        & 0.8754    & 0.5379   & 0.2205 \\ \hline
% FID-TOD w/ API-descriptions   (N=1) & 1.653 & 0.8963 & 0.9914    & 0.6584        & 0.8735    & 0.5428   & 0.2178 \\ \hdashline
% FID-TOD w/ API-descriptions   (N=5) & 1.655 & 0.8973 & 0.9908    & 0.6634        & 0.8739    & 0.5450   & 0.2192 \\ \hline
% BART + Retriever                 & 1.683 & 0.8945 & 0.9909    & 0.6533        & 0.8718    & 0.5425   & 0.2145 \\ \hdashline
% FiD-TOD                          & 1.676 & 0.8968 & 0.9913    & 0.6604        & 0.8726    & 0.5440   & 0.2172 \\ \hline
% \end{tabular}}\caption{Development results on SGD. By default, the retrieval module will retrieve Top-5 slot information entries from the cache.} \label{tab:tod-ablation}
% \vspace{-1.0em}
% \end{table*} 

\begin{table*}[]
\centering
\resizebox{0.98\linewidth}{!}{
\begin{tabular}{l|cccccc}
\hline
                                 & PPL   & JGA    & Unseen JGA & Token ACC & Token EM & BLEU-4 \\ \hline
BART-Large                       & 1.700 & 0.876    & 0.586        & \textbf{0.875}    & 0.538   & \textbf{0.221} \\ \hline
FID-TOD w/ API-descriptions   (N=1) & \textbf{1.653} & 0.896     & 0.658        & 0.874    & 0.543   & 0.218 \\ \hdashline
FID-TOD w/ API-descriptions   (N=5) & 1.655 & \textbf{0.897}    & \textbf{0.663}        & 0.874    & 0.544   & 0.219 \\ \hline
BART + Retriever                 & 1.683 & 0.895   & 0.653        & 0.872    & 0.543   & 0.215 \\ \hdashline
FiD-TOD                          & 1.676 & \textbf{0.897}   & 0.660        & 0.873    & \textbf{0.545}   & 0.217 \\ \hline
\end{tabular}}\caption{Development results on SGD. By default, the retrieval module will retrieve Top-5 slot information entries from the cache.} \label{tab:tod-ablation}
\vspace{-0.5em}
\end{table*} 





\section{Experimental Results}\label{sec:exp-results}


\paragraph{End-to-End TOD Performance}
Table \ref{tab:tod-main_results} shows the overall performance on the test set. FiD-TOD outperforms BART-Large on most metrics. Specifically, it improves the essential NLU metric, \textit{i.e.},  Unseen JGA, by  $6.7\%$, thus showing improvements on the unseen domains. The other metrics related to NLG are also slightly improved. 
% We emphasize that 
% due to GPUs resources limits at the later stage of the project in school, 
% we only fine-tune the retrieval module to retrieve correct slot information entries for the APICALL generation. 
Note that in this work we mainly focus on generating APICALLs, thus we only fine-tuned the retrieval module for APICALL generation and did not optimize the retrieval module to retrieve slot entries for the system response generation, \textit{i.e.}, there are noises introduced to the system response generation. We conjecture that we could continue to improve the NLG performance with a further fine-tuned retrieval module for system response generation. We leave the evaluation of NLG on purely unseen domains as future work.


\paragraph{Retrieval Performance}

We hope the model could generalize well since there could be lots of new  intents and slots in real scenarios. 
% more than half of the services and slots are unseen on the test set. 
Table \ref{tab:DPR} shows the Top-5 retrieval accuracy on the test set. We can see that the model handles well both seen and unseen intents and slots. It has good Top-1 accuracy and above $96\%$ Top-5 accuracy. Compared to only using names, adding related service and intent descriptions improves the Top-1 accuracy by more than $5\%$, which indicates that adding descriptions could help the model generalize to new unseen domains and services. 
Regarding the ``API-descriptions'', where a single entry in the cache includes all intents and slots information for the whole dialogue. We see that the model has good Top-1 accuracy and high Top-5 accuracy, \textit{i.e.}, the model has a high potential to retrieve all the related intents and slots information through single-time retrieval. Besides, we test some other templates, such as switching orders of intents and slots, and we find no significant differences. We also find that adding the special tokens ``INTENT'' and ``SLOT'' slightly deteriorates the Top-1 accuracy. 

We experiment with both normal negative and hard negative pairs, including different numbers of hard negative pairs, and we do not find significant differences in w.r.t retrieval performance. One potential reason is that the number of candidates in the cache is pretty tiny, \textit{i.e.}, the number of queries (dialog history) is much larger than the number of candidates. Consequently, the DPR model is easily overfitting upon one epoch training. 
 
\paragraph{Performance of Variants of Cache on End-to-End TOD}
% We design various templates for the cache
% , where the information entries in the cache are retrieved by the retrieval module and incorporated into the end-to-end TOD. 
Since we designed various templates for the cache, we want to test the influence of various cache templates on the end-to-end TOD. Table ~\ref{table:variants-of-db} shows that FiD-TOD with only using names is already much better than BART-Large, and adding descriptions could further improve the performance, \textit{e.g.}, ``\textit{INTENT: intent name, service description, intent description, SLOT: slot name, slot description}'' outperforms BART-Large and ``\textit{INTENT: intent name, SLOT: slot name}'' by $7.4\%$ and $2.7\%$ on Unseen JGA, respectively. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[]
\resizebox{\linewidth}{!}{
\begin{tabular}{l|l}
\hline
...                                         &  ...                                                                                                                                                                                                                            \\ \hline
SYSTEM:                                     & Do you want to make a reservation for 2 people in the restaurant?                                                                                                                                                                                          \\ \hline
USER:                                       & Yes, thanks. What’s their phone number?                                                                                                                                                                                                                    \\ \hline
                                            & \begin{tabular}[c]{@{}l@{}}INTENT: ReserveRestaurant , a popular restaurant search and reservation service ,  make \\ a table reservation at a restaurant , SLOT: {\color[HTML]{00D2CB} number\_of\_seats} , number of seats to reserve at the restaurant\end{tabular}            \\ \cdashline{2-2} 
                                            & \begin{tabular}[c]{@{}l@{}}INTENT: ReserveRestaurant ,  a popular restaurant search and reservation service ,  make \\ a table reservation at a restaurant ,  SLOT: time , tentative time of restaurant reservation\end{tabular}                           \\ \cdashline{2-2} 
                                            & \begin{tabular}[c]{@{}l@{}}INTENT: ReserveRestaurant ,  a popular restaurant search and reservation service ,  make \\ a table reservation at a restaurant , SLOT: date , tentative date of restaurant reservation\end{tabular}                            \\ \cdashline{2-2} 
                                            & \begin{tabular}[c]{@{}l@{}}INTENT: ReserveRestaurant ,  a popular restaurant search and reservation service ,  make \\ a table reservation at a restaurant , SLOT: restaurant\_name,  name of the restaurant\end{tabular}                                  \\ \cdashline{2-2} 
\multirow{-5}{*}{\begin{tabular}[c]{@{}l@{}}RETRIEVAL: \\ (Predicted Top-5)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}INTENT: ReserveRestaurant, a popular restaurant search and reservation service ,  make \\ a table reservation at a restaurant , SLOT: {\color[HTML]{00D2CB} location} , city where the restaurant is located\end{tabular}                              \\ \hline
APICALL: (Gold)                             & \begin{tabular}[c]{@{}l@{}}api\_name = ReserveRestaurant ; date = 2019-03-01 ; {\color[HTML]{00D2CB} location} = San Jose ; {\color[HTML]{00D2CB} number\_of\_seats} = 2 ; \\ restaurant\_name = Sino ;  time = 11:30\end{tabular}                                                                       \\ \hline
APICALL: (Predicted)                        & \begin{tabular}[c]{@{}l@{}}api\_name = ReserveRestaurant ; date = 2019-03-01 ; {\color[HTML]{CB0000} city} = San Jose ; {\color[HTML]{CB0000} party\_size} = 2 ; \\ restaurant\_name = Sino ; time = 11:30\end{tabular}                                                                                 \\ \hline
APIRESP:                                    & \begin{tabular}[c]{@{}l@{}}city = San Jose ; cuisine = Asian ; has\_live\_music = False ; phone\_number = 408-247-8880 ;  \\ price\_range = moderate ;  restaurant\_name: Sino;  serves\_alcohol = False ;  street\_address = 377 Santana Row\end{tabular} \\ \hline
SYSTEM:                                     & The phone number is 408-247-8880.                                                                                                                                                                                                                          \\ \hline
\end{tabular}} \caption{A predicted example on the development set. Red colors indicate incorrect predictions and light blue colors indicate correct slots. } \label{tab:error_analysis}
 \vspace{-0.5em}
\end{table*}


\paragraph{Influence of Irrelevant Information on the End-to-End TOD}
% In real scenarios, one cannot expect a perfect retrieval module as it could retrieve irrelevant or incorrect information from the cache. To test whether the generator can learn to make a balance between the dialog history and the grounded retrieved slots and whether it can learn to ignore irrelevant information. \textcolor{red}{->Put to another place}}
As many emerging and unseen intents and slots could appear in real scenarios,  it is thus hard to expect a perfect retrieval module. In this section, first, we investigate ``\textit{the TOD's ability in learning to ignore irrelevant retrieved information}''. 
% In this section, we first to investigate the ``\textit{influence to the End-to-End TOD if we give more irrelevant information to the Generator}''.
Table \ref{tab:tod-ablation} shows the corresponding results. As described in Sec \ref{section-cache}, ``\textit{API-descriptions}'' includes all intents and slots for the whole dialogue, and the retrieval module has $84.4\%$ Top-1 accuracy to retrieve all the slot information in a single time as shown in Table \ref{tab:DPR}. In addition, Top-5 accuracy measures whether the gold values appear on the Top-5 retrieved slot entry candidates. If we set $N$ to 5, the retriever will return similar but irrelevant information, even though the Top-5 accuracy is around $100\%$. Thus it will incorporate several irrelevant intents and slots. However, we find that ``\textit{API-descriptions (N=1)}''  performs similar to \textit{API-descriptions (N=5)}, as shown in row 2 and row 3 of Table \ref{tab:tod-ablation}. It indicates that the TOD can learn to ignore irrelevant retrieved information.

% \textcolor{blue}{Questions: What are the messages from other rows?}
Second, we investigate ``\textit{whether the TOD generator ground more on the retriever if we stack all retrieved information together}''. Here we compare ``BART+retriever'' and FiD-TOD, and their difference is on whether we handle the retrieved information entries together or separately. Row 3 in Table~\ref{tab:tod-ablation} shows that ``BART+retriever'' performs slightly worse after stacking the retrieved slots together. This finding indicates that the generator may not be able to ground more on the retriever even if we directly put all the retrieved information into the dialog history.  

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


\paragraph{Error Analysis}
The retriever module has a reasonably good Top-5 accuracy, whereas the  JGA is still far from perfect. We are thus curious what are the potential reasons. 
Table \ref{tab:error_analysis} shows one most frequently appeared error type, where the retrieval module could correctly retrieve Top-5 slot information entries from the cache. Regarding the APICALL prediction, the TOD correctly generates  the intent and values. Among the generated slots,``\textit{city}'' and ``\textit{party\_size}''  are semantically similar to  ``\textit{location}'' and ``\textit{number\_of\_seats}'', respectively. However, the two generated slots are incorrect as they are from different services, and with further check, we find that they are from the training cache. Which suggests that the TOD generator does not fully trust the retriever, and it just memorizes the training slot information entries in the training cache and requires more generalized ability. Moreover, we found there are around $20\%$ dialogue turns with this issue on the development set, indicating a huge space to further improve the performance.  We conjecture that data augmentation, such as entity replacements on dialog history,
could be one possible way to mitigate this issue.
% and improve performance. 
% Another possible way is dynamically updating the training cache during the training process. 
We leave more study as the future work. 

\paragraph{Limitation}  Our approach needs better retrieval modules to handle very limited intents and slots, as the retrieval module is easy to overfit in such scenarios. It also requires further designs for both the cache and the framework to integrate retrieved information from the large-scale cache, \textit{e.g.}, the internet or large-scale knowledge bases, into the end-to-end TOD systems. Besides, compared with the broad deployments of conventional pipeline-based TOD systems in the industry, end-to-end TOD systems are mainly developed from the research perspective. We may encounter issues when deploying end-to-end TOD systems into real industry scenarios. 







==> exp_settings_copy.tex <==


\section{Experimental Settings}
\subsection{Dataset}
 A substantial number of end-to-end TOD works~\citep{hosseini2020simple,peng2021soloist,lin2020mintl,yang2020ubar,su2021multi,he2022galaxy,feng2023fantastic} commonly employ the MultiWOZ datasets~\citep{budzianowski2018multiwoz,zang2020multiwoz}. However, these studies primarily focus on full-shot and few-shot learning, with less emphasis on zero-shot evaluation. This scope for zero-shot evaluation appears somewhat constrained given that MultiWOZ only has five domains and approximately $35$ slots, all of them are presented in the training set. In contrast, our work aims to assess the system across large-scale, unseen dialog domains. We utilize the  Google Schema-Guided Dialogue (SGD) dataset~\cite{rastogi2020towards}. SGD provides a more expansive dialog landscape, with  over $16$k multi-domain conversations across more than $16$ domains and $200$ slots. Importantly,  half of these domains and slots do not appear in the development and test sets.
\footnote{\url{https://github.com/google-research-datasets/dstc8-schema-guided-dialogue}}. 
Table~\ref{dataset:SGD} summarizes the statistics of SGD. 




\subsection{Models}\label{sec:labels}

Our end-to-end TOD framework's backbone models are compatible with most pre-trained generative models, \textit{e.g.}, GPT-2, T5, and BART. These models have been widely applied to settings of previous state-of-the-art approaches such as \cite{chen2020simple,lin2020mintl,su2021multi}. 

Regarding baselines, we follow  \cite{lin2020mintl,chen2021teaching} and implement their model MinTL (BART-Large),  and we follow \cite{lee2021dialogue} and implement T5DST, which achieves SOTA performance on MultiWOZ 2.2~\citep{zang2020multiwoz}.  Since our end-to-end TOD framework is compatible with existing pre-trained generative models, we experiment with BART, GPT2 and T5, and found that BART-Large (406M) performs similarly to T5-Large (770M) with less parameters and outperform SOTA models designed by teams in DSTC8~\citep{rastogi2020schema}, we thus treate BART-Large as a backbone model.

We follow them and run preliminary experiments on SGD, and we find that BART performs best compared with other pre-trained models with similar parameters. Besides, BART outperforms state-of-the-art models designed by 
teams on DSTC8~\citep{rastogi2020schema}, where most models are classification models based on BERT. We thus use the BART-Large model as a backbone and baseline model. 
% The BART-Large model's implementation process on TOD is similar to \citep{lin2020mintl,chen2021teaching}.
The implementation process of the BART-Large model is similar to that of \citep{lin2020mintl,chen2021teaching} on TOD.
In addition, previous work~\cite{peng2021soloist,su2021multi, he2022galaxy} first pre-train models on several task-oriented dialogue datasets or multi-task learning. We only train the model on the SGD dataset, and instead of  claiming state-of-the-art performance, our goal is to validate our proposed approach. 

\begin{table}[]
\resizebox{\linewidth}{!}{
% \begin{tabular}{l|l|l|l|l|l}
\begin{tabular}{l|ccccc}
 \hline
            & Dialogues & Domains & Services & ZS Domains & ZS Services \\ \hline
Train       & 16142     & 16      & 26       & -                 & -                  \\
Dev. & 2482      & 16      & 17       & 1                 & 8                  \\
Test        & 4201      & 18      & 21       & 3                 & 11              \\  \hline
\end{tabular}}\caption{Data Statistics of SGD. ZS: Zero-Shot.}\label{dataset:SGD}
\end{table}


\begin{figure}%[t]
	\begin{center}
    % 	\includegraphics[width=\linewidth]{./images/Confusion_Matrix-Roberta.png}
    	\includegraphics[width=\linewidth]{./images/Fid_rag.png}
    \end{center}
    %\vspace{-1.5em}
\caption{Illustration of the end-to-end FiD-TOD framework with a simple cache. Here we show the system response generation process, and the APICALL generation process is similar to that in Figure \ref{fig:tod_framework}. 
}
\label{fig:tod_framework_2}
% \vspace{-0.8em}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table*}[]
% \centering
% \resizebox{0.98\linewidth}{!}{
% \begin{tabular}{l|ccccccc}
% \hline
%         & PPL            & JGA             & Empty JGA       & Non-Empty JGA   & Token ACC      & Token EM        & BLEU-4 \\ \hline
% BART-Large    & 2.385          & 0.8119          & \textbf{0.9901} & 0.3643          & 0.8365          & 0.4970          & \textbf{0.1786} \\
% FiD-TOD & \textbf{2.133} & \textbf{0.8293} & 0.9878          & \textbf{0.4310} & \textbf{0.8393} & \textbf{0.5013} & 0.1785 \\ \hline
% \end{tabular}}\caption{Testing results on the SGD dataset. } \label{tab:tod-main_results}
% \end{table*}

\begin{table*}[]
\centering
\resizebox{0.98\linewidth}{!}{
\begin{tabular}{l|cccccc}
\hline
        & PPL            & JGA                  & Unseen JGA   & Token ACC      & Token EM        & BLEU-4 \\ \hline
BART-Large    & 2.385          & 0.812           & 0.364          & 0.837          & 0.497          & \textbf{0.179} \\
FiD-TOD & \textbf{2.133} & \textbf{0.829}       & \textbf{0.431} & \textbf{0.839} & \textbf{0.501} & \textbf{0.179} \\ \hline
\end{tabular}}\caption{Testing results on the SGD dataset. } \label{tab:tod-main_results}
\end{table*}
% The cache of FiD-TOD uses the second template in Table \ref{table:cache}.
%Note that due to the end of my internship at an anonymous company, company legal rules forbid copying any checkpoints and minimal GPU resources to rerun configured experiments in school. I report the development results of more models on the following tables.

\begin{table*}[]
\centering
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{l|ccccc}
\hline
Cache Templates                                                                                                                               & Top-1           & Top-2           & Top-3  & Top-4  & Top-5  \\ \hline
INTENT: intent name, SLOT: slot name                                                                                               & 0.833 & 0.882 & 0.914 & 0.945 & 0.960 \\ \hdashline
\begin{tabular}[c]{@{}l@{}}INTENT: intent name,  service description, \\ intent description, SLOT: slot name, slot description\end{tabular} & 0.887 & 0.922 & 0.952 & 0.976 & 0.980 \\ \hline
intent name, slot name, intent description, slot description                                                                                         & 0.835 & 0.906 & 0.928 & 0.946 & 0.955 \\ \hdashline
\begin{tabular}[c]{@{}l@{}}intent name, slot name, service description, \\ intent description, slot description\end{tabular}                         & 0.913 & 0.943 & 0.965 & 0.977 & 0.981 \\ \hline
API-descriptions                                                                                                                      & 0.844 & 0.927 & 0.956 & 0.962 & 0.967 \\ \hline
\end{tabular}} \caption{Top-5 retrieval accuracy on the test set of SGD. } \label{tab:DPR}
\vspace{-0.8em}
\end{table*}

We fine-tune the retrieval module up to 3 epochs based on open-sourced DPR~\citep{karpukhin2020dense}.
% \footnote{\texttt{\url{https://github.com/facebookresearch/DPR}}}. 
We run our experiments based on the ParLAI platform~\citep{miller2017parlai}, where we rely on publicly available code of the BART model and the FiD-RAG model\footnote{\texttt{\url{https://github.com/facebookresearch/ParlAI/tree/main/parlai/agents/rag}}}. The FiD model and RAG model originally come from~\cite{lewis2020retrieval,izacard2021leveraging}. By default, we use the RAG-Turn Token setting~\cite{shuster2021retrieval} for the RAG model.  
We design two variants for end-to-end TOD systems: the first variant, termed FiD-TOD, is based on the FiD-RAG model,  as shown in Figure~\ref{fig:tod_framework_2}. The second variant is ``BART+Retriever'', as illustrated in the previous Figure~\ref{fig:tod_framework}. FiD-TOD is the same as the ``BART+Retriever`` model, except that the dialog history with each retrieved slot entry are concatenated and sent to the shared encoder. After that, all information are merged and sent to the decoder to generate the APICALL and the system response. The retrieval module and the TOD generator can be trained jointly~citep{lewis2020retrieval} or separately~\citep{lewis2020retrieval,izacard2021leveraging,shuster2021retrieval}. 
% In our work, we train them separately as we found that compared with jointly training, it could stabilize the training process and improve performance. 
In our work, we follow settings in open-domain conversations and train them separately to enhance flexibility to the TOD system. 

Similar findings are also found in open-domain question answering and open-domain conversations~\citep{lewis2020retrieval,izacard2021leveraging,shuster2021retrieval}. 

We retrieve Top-5 slot information entries from the cache and truncate the tokens of dialog history to 256, unless otherwise stated.  We align one hard negative pair to each positive pair for the DPR fine-tuning.  We followed the ParLAI code's preset hyper-parameters, such as learning rate to 5e-5, batch size to 32, etc., and did not optimize them. 
We fine-tune the end-to-end auto-regressive TOD model (770M) up to 4 epochs with an overall batch size of $64$ on $8$ NVIDIA Tesla V100 GPUs, where each GPU has 16GB memory.  The training process takes around 8 hours. 






\subsection{Evaluation Metrics}

We evaluate the end-en-end TOD framework using the following metrics: (1) Top-$N$ accuracy: It evaluates the retrieval module through checking whether the ground-truth slot appears in the Top-$N$ predicted candidates~\cite{karpukhin2020dense}. (2) Joint Goal Accuracy (JGA): It evaluates whether the predicted APICALL on both seen and unseen domains is correct or not, specifically. JGA is $1$ if the model correctly predicts all intent, slots and corresponding values in the APICALL. Otherwise, JGA is $0$. 
% (3) Empty JGA: As many dialogue turns do not involve an APICALL, \textit{i.e.}, the APICALL is empty, we employ Empty JGA to evaluate whether the model should trigger an API retrieval.   
% (4) Non-Empty JGA: It evaluates whether JGA is correct if the model calls the API. As most dialogue turns have empty APICALL and identifying Empty JGA is relevantly easy, we treat Non-Empty JGA as the most crucial metric for JGA. 
(3) Unseen JGA: It evaluates whether JGA is correct if the model calls the API on unseen domains. In SGD, most dialogue turns would not trigger an API retrieval, resulting in empty APICALLs, and identifying Empty JGA is relatively easy~\citep{chen2021teaching}. Therefore, we focus on non-empty APICALL turns and treat Unseen JGA as the most crucial metric on unseen domains.
(4) Token EM:  It evaluates the utterance-level token accuracy. Roughly corresponds to perfection under greedy search (generative only). (5) Perplexity (PPL) and Token ACC: Both measure the generative model’s ability to predict individual tokens. PPL measures perplexity, and Token ACC measures the per-token accuracy. (6) BLEU-4: It measures the BLEU score~\cite{papineni2002bleu} between the predicted system response and the reference response.  
 \footnote{Most metrics can be found in \url{https://parl.ai/docs/tutorial_metrics.html}.}












==> introduction_old.tex <==
\section{Introduction}

% I am training a T5-large model and T5-3B model to predict system response based on prompt, previous dialog context and noisy external knowledge. Since in real scenarios, the customers may have different input, to simulate such situations. I have 10m examples, and i want 80% data with normal order, and the rest 20% data with commonly used other orders from customers. And i also add variations for the special tokens, such as instruction_tokens = ["Instruction:", "Prompt:", "Task:", ""], ek_tokens = ["External Knowledge:", "External Information:", "Supplementary Information:", "Other Knowledge:"]                         dialog_input_tokens = ["Input:", "Dialog Input:", "Dialog history:", "Conversation History:",  "Dialog Context:"] What are your suggestions to me? 

% Default order: 
%     Dialog, Prompt, Ek 
% Other orders:
%     Prompt, Dialog, EK 
%     Prompt, EK, Dialog 
%     Dialog, EK, Prompt 


% Currently, we utilize 18 datasets with the default order and the rest with various orders. To make the model more robust, we also add variations towards the separator tokens.


% Task-oriented dialog (TOD) systems, which are able to assist humans in finishing various tasks such as booking restaurants, setting alarms, and making recommendations, have played an important role in daily life~\cite{gao2018neural}. 
Task-oriented dialog (TOD) systems, as assistant tools in various tasks such as restaurants booking, alarm setting, and recommendations, have played an important role in daily life~\cite{gao2018neural,xie2022converse}.
% There are two types of TOD systems: pipeline-based dialog system and end-to-end dialog system. 
Currently, the TOD systems can be categorized into two groups: pipeline-based dialog systems, and end-to-end dialog systems.
% Pipeline-based dialog system includes four different modules, i.e., natural language understanding (NLU) to understand user intents, dialog state tracking (DST) to track user belief state across dialog turns, dialog management (DM) to decide the system action for interacting with users based on the dialog state, and natural language generation (NLG) to maps system actions to natural language responses. 
The pipeline-based dialog systems consist of four different modules, \textit{i.e.}, a natural language understanding (NLU) module to detect user intents, a dialog state tracking (DST) module to track the belief states of users across dialog turns, a dialog management (DM) module to carry out the system actions to interact with users based on the dialog states, as well as a natural language generation (NLG) module to generate natural-language responses for users. 
However, building such pipeline-based systems is label-intensive, error-propagated, and hard to scale~\cite{hosseini2020simple, peng2021soloist}. 
\begin{figure}%[t]
	\begin{center}
    	\includegraphics[width=1.0\linewidth]{./images/main_example.png} %new_example
    \end{center}
    %\vspace{-1.5em}
\caption{An example of the auto-regressive TOD. We mainly show the APICALL generation process here, and the system response generation process is similar. 
% RETRIEVAL module retrieves slot information entries from the cache. APICALL is identical to the dialog state. APIRESP returns information from external API interactions between the system and system databases. 
Here $N$ is set to 3 for the retrieval module.  
% An example for the auto-regressive TOD. The example includes the first three turns of a dialog. The TOD generates the APICALL and system response. Then it automatically gets the APIRESP  from the original system database based on the APICALL. APIRETRIEVAL returns retrieved slot information from the simple constructed cache, and it returns top-N slots and combines them based on a template. In this example,  we set $N$ to 3. 
}
\label{fig:example_tod}
%  \vspace{-0.5em}
\end{figure}

% Recently, 
% % there has been a lot of success with
% much progress has been made on using pure seq2seq language models in order to alternate between structured output and NLG in end-to-end TOD systems, and these systems~\cite {ham2020end,lin2020mintl,yang2020ubar,gao2021hyknow,chen2021teaching,peng2021soloist,liu2021pretraining,he2022galaxy} outperform pipeline-based methods on public datasets.
Recently, various approaches have been proposed to generate the dialog states and responses based on seq2seq models, in an end-to-end manner~\cite {ham2020end,lin2020mintl,yang2020ubar,gao2021hyknow,chen2021teaching,peng2021soloist,liu2021pretraining,he2022galaxy}.
% They require less direct annotations, e.g., no dialog acts, no intents, only dialog states, and natural language response, and promise to leverage pre-trained models' sophisticated NLU and NLG capabilities. 
% These methods have been shown to be effective when compared with the pipeline-based methods on several public datasets, with fewer annotations such as dialog acts, and user intents.
Compared with the pipeline-based methods on public datasets, these methods show effectiveness, with fewer direct annotations such as user intents and dialog acts. 
Moreover, they can easily benefit from the strong capabilities of large-scale pre-trained language models (\textit{e.g.}, GPT-2~\citep{radford2019language}, T5~\citep{raffel2019exploring} and BART~\cite{lewis2020bart}) in NLU and NLG.
% In general, they have the following patterns: 
% From our investigation, current seq2seq-based approaches for TOD systems generally follow the following patterns:
% (1) Rely on powerful pre-trained seq2seq models. (2) Directly use language modeling objective to generate NLU and NLG, or add auxiliary goals such as DST loss. (3) Directly fine-tune models on the target dataset or conduct pre-training on several TOD dialogue datasets first. (4) Design or adopt data augmentation techniques such as entity replacement to augment training dialogues. 
% such as back-translation and entity replacement to improve performance due to the laboriousness to collect many TOD dialog corpora. 
% Although previous works have achieved impressive performance in end-to-end TOD systems, 
% \textcolor{blue}{the interactions with the system database do not help a lot to improve NLU and NLG}~\cite{hosseini2020simple}.  Moreover, previous systems
However,
they 
% have limited capabilities, especially 
are limited in the
the flexibility of dynamically handling existing, unseen, or emerging intents and slots~\cite{hosseini2020simple,peng2021soloist}.

% Meantime, 
% % there has been a lot of initial success 
% there have been several attempts to augment generative models with the retrieved information. 

% \textcolor{blue}{
% To xxxx, 
Additionally, 
% several attempts have been made 
another direction of work aims
to augment the generative models with retrieved information in open-domain question answering and open-domain dialog systems. 
In particular, these models first retrieve information related to the question or user query from a database of sentences or passages, then incorporate such information into the models to generate answers~\cite{karpukhin2020dense,izacard2021leveraging} or open-domain dialog responses~\cite{dinan2018wizard,lewis2020retrieval,shuster2021retrieval}.
% on using retrieval augmented generation models which are able to retrieve from a database of sentences or passages and provide answers for questions~\cite{karpukhin2020dense} or ground the generation response on the retrieved information~\cite{dinan2018wizard,lewis2020retrieval,shuster2021retrieval,izacard2021leveraging}. 

% \textcolor{blue}{Yao: the motivation of our work is weak. Why simple cache? What is the insight?
% xxx motivate us to introduce a simple cache to xxxxx, inspired by the temporal storage in computer architecture.
% Figure 1 shows a motivating example of our approach.
% Overall, the following two paragraphs should be strengthened.
% }
In this paper, we combine  both worlds into an end-to-end TOD system. 
% We train end-to-end TOD models with a simply designed cache, and the cache includes all the accessible intents, slots, or other information from the dataset. 
We train the end-to-end TOD models by introducing a simply designed cache containing all the accessible intents and slots from the dialogues.
% The model 
Our approach can reference and ground the retrieved information from the cache while performing TOD. Figure~\ref{fig:example_tod} shows a motivating example of our approach, in which the RETRIEVAL module retrieves slot information from the cache. APICALL is identical to the dialog states from the system side. APIRESP returns information from external API interactions between the system and system databases.
% \textcolor{blue}{Yao: By using Figure 1, we should introduce what is cache, APICALL, and APIRESP.}
The cache could be decoupled from the actual inference, and it has the flexibility to be dynamically updated to add new intents and slots without intensive retraining. The flexibility would also be helpful to find and disable the wrong predicted slots in the future. 

% To achieve this goal, 
To build an accurate end-to-end TOD system with a simple cache, 
% we design a simple cache with intent and slot information, and we also add corresponding descriptions to enable better zero-shot generalization ability. In particular,
we first fine-tune a retrieval module to retrieve Top-$N$ slot information entries from the cache. Then    we plug it into generative models to help perform end-to-end TOD generation. 
% During this progress, we will only train the generative models and not update the parameters of the retrieval module.   
% \textcolor{blue}{
% We then xxxxx.
% }
We conduct experiments on the large-scale publicly available Google Schema-Guided Dialogue dataset (SGD)~\cite{google-schema-guided} with around half unseen intents and slots in the development and test set to verify the effectiveness of our approach.
% show our model outperforms strong baselines. validate the effectiveness of our model when compared with several strong baselines.

The contributions of this paper are as follows: (1) We design a simple yet effective end-to-end TOD framework with a simply designed cache where the backbone models are compatible with existing pre-trained generative models. (2) Our approach allows the model to dynamically disable existing or add new intents and slots without intensive retraining.
(3) Experimental results demonstrate the superior performance of our approach when compared with strong baselines. 
% (4) We conduct detailed ablation studies and analyses to facilitate future research on end-to-end TOD.
(4) We conduct extensive ablation studies and analyses to facilitate further research on building accurate end-to-end TOD systems.

% \begin{itemize}
% \item We design a simple end-to-end TOD framework with a simple cache. The backbone models are compatible with existing pre-trained generative models. \item The framework has the flexibility to dynamically update the cache to disable existing or add new or unseen domains, slots, APIs, etc., without intensive retraining.
% \item Experimental results demonstrate the superior performance of our model when compared with baselines. 
% \item We conduct detailed ablation studies and analyses to facilitate future research on end-to-end TOD.
% \end{itemize}






==> methodology_copy.tex <==
% \section{Task Definition for Few-Shot Intent Detection}

% and GPT-3~\citep{brown2020language}


\section{TOD Systems with a Simple Cache}
% In this section, we will 
Here we present the end-to-end framework with a simple cache, where we build our framework based on BART.
% , and other generative models such as GPT-2 and T5 could also be directly used as backbone models in our framework. 
In our framework, several generative models such as GPT-2 and T5 could also be directly used as backbone models.
% Figure~\ref{fig:example_tod} shows an example. 
Generally, our framework comprises two parts: the first part is a retrieval model for retrieving slot information entries from the cache; the second part is an end-to-end TOD that generates APICALLs and system responses based on the dialog history and the retrieved slot information.
Figure~\ref{fig:tod_framework} demonstrates one simple variant of our framework, \textit{i.e}. ``BART+Retriever'', where the retrieved slot information entries are stacked together. We also design the other variant ({\textit{i.e.}, ``FiD-TOD''}) in Sec.~\ref{sec:labels}, where each retrieved slot is concatenated with the dialog history and then all the information are concatenated together and sent to the decoder.  Figure~\ref{fig:tod_framework_2} shows the ``FiD-TOD'' model. To better illustrate the framework, we list the simpler ``BART+Retriever'' in the main figure and this section. 

% Figure~\ref{fig:tod_framework_2} shows the other variant, \textit{i.e.}, ``FiD-TOD''. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}%[t]
	\begin{center}
    % 	\includegraphics[width=\linewidth]{./images/Confusion_Matrix-Roberta.png}
    	\includegraphics[width=\linewidth]{./images/main_framework.png}
    \end{center}
    %\vspace{-1.5em}
\caption{Illustration of the end-to-end framework with a simple cache. The left part is an intermediate step of the right part, indicating the process of generating an APICALL. The right part is the process of producing a system response. In general, based on the dialog history, the retrieval module retrieves slot information entries from the cache. The dialog history and the retrieved information are sent to the decoder to generate the APICALL. The system continues to retrieve from the cache based on all previous information, and finally, it generates a system response.  
% \color{red}{Require better figures for a straightforward understanding, such as table \ref{tab:error_analysis}}
}
\label{fig:tod_framework}
%  \vspace{-0.5em}
\end{figure*}


\begin{table*}[]
\resizebox{\linewidth}{!}{
\begin{tabular}{ll}
\hline
Cache Templates                                                                                        & Examples                                                                                                                                                       \\ \hline
INTENT: intent name, SLOT: slot name                                                                                  & INTENT: findrestaurants, SLOT: city                                                                                                                                          \\ \hdashline
% {[}INTNET{]} intent name {[}SLOT{]} slot name & [INTENT] findrestaurants [SLOT] city  \\ \hdashline
\begin{tabular}[c]{@{}l@{}}intent name, slot name, service description, \\  intent description, slot description\end{tabular} & \begin{tabular}[c]{@{}l@{}}findrestaurants, city, a leading provider for restaurant search and reservations, \\  find a restaurant of a particular cuisine in a city, city in which the restaurant is located\end{tabular} \\ \hdashline
latest API-descriptions                                                                                  & \begin{tabular}[c]{@{}l@{}}api\_name = FindRestaurants; optArg = has\_live\_music, price\_range, \\ serves\_alcohol; reqArg = city, cuisine\end{tabular}       \\ \hline
\end{tabular}}\caption{Several typical templates of the simple cache construction, where each template represents one type of cache. With regard to the ``latest API-descriptions'', ``api\_name'' denotes the intents for the whole dialogue, and ``optArg'' and ``reqArg'' are all relevant slots in the whole dialogue. Some other templates can be found in Table \ref{tab:DPR}.}\label{table:cache}
\end{table*}

\subsection{Construction of Simple Cache}\label{section-cache}
As aforementioned, a cache of domains and slots can benefit models' referencing and grounding procedure when performing TOD generation.
% We want to train models which have a simple cache of slots names or other information which the model can reference and ground on while it is performing TOD generation.
To this end, we first build a simple cache, which includes names of intents and slots from accessible dialogues. Note that we give the name `cache' from a traditional computer CPU memory storage perspective to show that our cache is simple and easy to update. It is also easier to construct than the dataset `database' designed by the dataset constructors~\citep{budzianowski2018multiwoz,rastogi2020towards} and used by \citep{hosseini2020simple},  as the `database' includes every detail of individual intent, intent values, slots, slot values, locations, etc. 

% Explicitly, it incorporates the intents and slots information from training dialogues during training process, and it includes corresponding information 
% from the development/test set in the development/test phase. 
Explicitly, it contains all intents and slots from the accessible training dialogues, and its contents can be updated during training and inference. We will fine-tune a retrieval module to retrieve relevant information given a dialogue turn.
Table~\ref{table:cache} illustrates several templates for the cache construction. Specifically, we design ``latest API-description'' as one type of cache. It includes all the intents and relevant slots throughout the whole  dialogue; as such, it contains redundant information because when the conversation
% hasn't 
is not finished, a dialogue turn may only involves a few active intents and slots, and most intents and slots are not mentioned. Thus it helps us evaluate whether a model is able to learn to ignore irrelevant information. Except the typical listed templates in Table~\ref{table:cache}, we also design several other templates with special tokens such as ``\textit{[INTENT] intent name [SLOT] slot name}'', as well as those with different orders of intents and slots such as ``\textit{intent name, intent description, slot name, slot description}'' and ``\textit{intent name, slot name, intent description, slot description}''. 
% The effects of different types of cache will be discussed in the experimental part. 
We also discuss the effects of different types of cache in the experimental part. 
\subsection{Retrieval Module}

Given a dialog history $c$, the TOD system will trigger a retrieval module to retrieve Top-$N$ slots $s_1,\ldots, s_N$ from the cache. In detail, based on the user dialog history,  the system first calls the retrieval module to generate an APICALL which includes relevant active intents, slots and values. After that, the system continues to trigger the retrieval module to generate a system response based on all previous information. 

To correctly retrieve information from the cache, we fine-tune a dense passage retriever (DPR) model~\citep{karpukhin2020dense}, which is a BERT-based dual-encoder framework optimized via contrastive learning. Specifically, we yield the hidden representation $\mathbf{h}_c$ for the dialog history through an encoder model, \textit{e.g.}, $\mathbf{h}_c=\text{BERT}_c(c)$. We use another BERT encoder to get the feature representation $\mathbf{h}_{s}$ for a slot information entry of the cache, \textit{i.e.}, $\mathbf{h}_{s}=\text{BERT}_s(s)$. We measure the similarity between the dialog history and the information entry as: $sim(c, s)=\mathbf{h}_c^{T}\odot\mathbf{h}_{s}$.
There are $n$ relevant (positive) entries and $m$ irrelevant (negative) entries given one dialog history, where $n$ and $m$ may vary as each dialog history would contain different active slots. 
We aim to learn a function to minimize the distance between the pairs of relevant dialog history and slot information entries than the irrelevant pairs. Given a specific pair, the corresponding loss function is as follows:
\begin{equation}
    \label{eq:hard-negative-eq}
    \small
    \mathcal{L}_{\text{api}}(c,s_{1}^{+},s_{1}^{-},\ldots, s_{m}^{-})=-\log\frac{\exp(\text{sim}(\mathbf{h}_c,\mathbf{h}_{s_{1}^{+}}))}{\sum_{j=1}^{m}\exp(\text{sim}(\mathbf{h}_c,\mathbf{h}_{s_{j}^{-}}))}\,.
\end{equation}

Once we finish fine-tuning the retrieval module, we will plug it into the end-to-end TOD generative model. The model parameters of the retrieval module will not be further updated when we train the generative model. 

% Note that we only optimize the retrieval module for generating correct APICALLs. Currently, we do not further fine-tune the retrieval module for generating better system responses, and 
% % we plan to optimize it in the future.
% we leave the optimization to our future work.

\paragraph{Negative Sampling} In a training batch, slot information entries irrelevant to the dialog history could naturally be formalized as negative pairs. To improve the robustness and performance of the retrieval module, we design some hard negative pairs. Instead of manually combining intents and slots; for instance, given a positive pair ``\textit{active intent, active slots}'', a natural negative pair could be ``\textit{inactive intent, inactive slots }''. We further construct hard negative pairs such as: ``\textit{active intent name, inactive slots from the same active intent}'' and ``\textit{inactive intents which are semantically similar to the active intents, active slots from the active intents}''. Another way is automatically selecting hard negative pairs during the training process. Specifically, we treat Top-$K$ ranked irrelevant slot entries from the cache as hard negative pairs.  Currently, we use the first way to conduct negative sampling and leave the second way to future work.



\subsection{End-to-End TOD Systems}
Our end-to-end TOD framework generates the APICALL and system response in an auto-regressive way. Figure~\ref{fig:example_tod} shows an example. The APICALL contains relevant intents, slots, and corresponding slot values, and it is similar to the dialogue belief states, although it focuses on the system side~\citep{chen2021teaching}.  Same with previous work~\citep{hosseini2020simple,peng2021soloist}, the APICALL is an intermediate step of the system response generation, and they share the same model framework and generate tokens autoregressively.    Given that a dialogue consists of several turns, the TOD framework triggers the retrieval module twice at a specific dialogue turn. The system first retrieves slot information entries from the simple constructed cache, \textit{i.e.},
\begin{equation}
    \small
\text{Top-$N$ slots} = \text{Retrieval}(c)\,.
\end{equation}
Then it generates an APICALL, \textit{i.e.}, 
\begin{equation}
    \small
\text{APICALL} = \text{TOD}(c, \text{Top-$N$ slots)}\,.
\end{equation}
After that it will continue retrieving another Top-$N$ slot information entries from the cache, \textit{i.e.}, 
\begin{equation}
    \small
\text{Top-$N$ slots} = \text{Retrieval}(c, \text{APICALL}, \text{APIRESP})\,,
\end{equation}
% $\text{retrieved top\_N slots} = \text{APIRetrieval}($c$, \text{APICALL}, \text{APIRESP})$, 
where the APIRESP is automatically yielded through an API interaction with the original system database when we have an active APICALL and it does not need to be predicted.  

Finally it generates a system response:
\begin{equation}
\small
% \begin{aligned}
    \text{Response} = \text{TOD($c$, APICALL, APIRESP, Top-$N$ slots)}\,.
% \end{aligned}
\end{equation}













==> miscs.tex <==

\section{Introduction}

Existing methods address the few-shot intent detection tasks mainly from two perspectives: (1) data augmentation and (2) task-adaptive training with pre-trained models. For the first category, \newcite{zhang2020discriminative} and \newcite{mehri2020example}  propose a nearest neighbor classification schema with full use of the limited training examples in both training and inference stages. 
% However, the model training is very expensive and hard to scale to tasks with several intents. 
% \citep{eda} proposes simple text editing rules such as insert and swap, and \citep{deng2019low} proposes back translation for data augmentation, while such methods have been shown not to work well on few-shot intent detection. 
\newcite{xia2020cg} and \newcite{peng2020data} propose to generate utterances for emerging intents based on variational autoencoder~\citep{kingma2013auto} and GPT-2~\citep{radford2019language}, respectively. 
% However, the generated utterances are noisy and require human filtering. 
For the second category,  \newcite{efficient_intent}  and \newcite{mehri2020dialoglue} conduct intent detection by leveraging related conversational pre-training models based on a few hundred million conversations.  Meanwhile, they devise a task-adaptive training schema where the model is pre-trained on all relative intent datasets or the target intent datasets with mask language modeling. 


However, previous methods such as data augmentation related models~\cite{liu2021augmenting} are inefficient for training and hard to scale to tasks with lots of intents. Moreover, these models do not tackle well the following scenarios: In real scenarios, the few-shot intent detection could be more challenging when there exist many fine-grained intents, especially semantically similar intents. For instance, BANKING77~\citep{efficient_intent} has a single domain with 77 intents, and CLINC150~\citep{oos-intent} has ten domains with 150 intents. 
Many intents in the datasets are similar. Therefore, training models is rather challenging when there are only limited examples. 

Inspired by the recent success of contrastive learning~\citep{he2020momentum,gunel2020supervised,chen2020simple,radford2learning,liu2021fast,gao2021simcse,liu2021contrastive}, which aims to enhance 
discrimination abilities of models,
% enforce examples from the same class close and the examples from different classes apart,
this work proposes improving few-shot intent detection via Contrastive Pre-training and Fine-Tuning (CPFT). Intuitively, we first learn to implicitly discriminate semantically similar utterances via contrastive self-supervised pre-training on intent datasets without using any intent labels. 
We then jointly perform few-shot intent detection and supervised contrastive learning. The supervised contrastive learning helps the model explicitly learn to pull utterances from the same intent close and push utterances across different intents apart. 

% We also notice some very recent works~\citep{liu2021fast,gao2021simcse,gunel2020supervised} adopting contrastive learning in natural language processing tasks. Our work differs them in: Firstly, we specifically tackle the few-shot intent detection task; Secondly, we employ contrastive  learning in both self-supervised pre-training and supervised fine-tuning stages.
% with two stages. 
% rather than general \textcolor{red}{single-stage contrastive pre-training or fine-tuning}. 
% We also do not need to specifically design and handle hard negative examples.

Our contributions are summarized as follows: 1) We design a simple yet effective few-shot intent detection schema via contrastive pre-training and fine-tuning. 2) Experimental results verify the state-of-the-art performance of CPFT on three challenging datasets under 5-shot and 10-shot settings.


\begin{table*}[]
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|cc|cc|cc}
\hline
                                                                  & \multicolumn{2}{c|}{CLINC150} & \multicolumn{2}{c|}{BANKING77} & \multicolumn{2}{c}{HWU64} \\
Model                                                             & 5-shot        & 10-shot       & 5-shot        & 10-shot       & 5-shot      & 10-shot      \\ \hline
CPFT                                                              & 92.34         & 94.18         & 80.86         & 87.20          & 82.03       & 87.13        \\ \hdashline
w/o Contrastive pre-training                                       & -4.15         & -2.63         & -4.11         & -2.37         & -6.01       & -4.17        \\
w/o Supervised contrastive learning                               & -0.56         & -0.32         & -2.06         & -0.88         & -1.14       & -0.27      \\
w/o Contrastive pre-training + w/o Supervised contrastive learning & -4.35         & -2.69         & -6.82         & -2.93         & -6.47       & -4.23        
  \\ \hline
\end{tabular}} \caption{Testing accuracy ($\times 100\%$) of CPFT with variants on three datasets under 5-shot and 10-shot settings.}\label{table:ablation-study}
% \vspace{-1em}
% \vspace{-5mm}
\end{table*}



\section{Experimental Results}


 We show  the overall comparisons on three datasets in Table \ref{table:main-results}. The proposed CPFT method achieves the best performance across all datasets under both the 5-shot and 10-shot settings. Specifically,  CPFT outperforms DNNC by 1.32\% and 1.57\% on CLINC150 and HWU64 under the 5-shot setting, respectively. It also improves DNNC by 2.41\% on HWU64 under the 10-shot setting. 
 Our variances are also lower when compared with DNNC: Ours vs. DNNC: 0.39 vs. 0.57 and 0.18 vs. 0.42 on CLINC150; 0.20 vs. 0.88 and 0.48 vs. 0.21 on BANKING77; 0.51 vs. 1.00 and 0.25 vs. 0.38 on HWU64 under 5-shot and 10-shot settings, respectively.
 The improvements indicate that our proposed method has a better ability to discriminate semantically similar intents than the strong discriminate nearest-neighbor model with data augmentation.
Moreover, the DNNC training is expensive, as when training models on a single NVIDIA Tesla V100 GPU with 32GB memory, DNNC takes more than $3$ hours for 10-shot learning on CLINC150, and it needs to retrain the model for every new setting. CPFT only needs $2.5$ hours for one-time pre-training, and the  fine-tuning only takes five minutes for each new setting.  
Compared with CONVBERT+MLM, which does a self-supervised pre-training with MLM on the intent detection datasets, CPFT improves the performance by 1.43\%, 3.21\%, and 2.61\% on CLINC150, BANKING77, and HWU64 under 10-shot setting, respectively. CPFL also outperforms CONVBERT+Combined, which further adds examples-driven training and specific transformer attention design. We contribute the performance improvements to contrastive learning, which help the model discriminate semantically similar intents. 



\section{Ablation Study and Analysis}
\paragraph{Is the schema with both stages necessary?}
We conduct ablation study to investigate the effects of self-supervised contrastive pre-training and supervised contrastive fine-tuning. Table \ref{table:ablation-study} shows the testing results of CPFT with model variants on three datasets. Experimental results indicate that both stages are necessary to achieve the best performance. The self-supervised contrastive pre-training on the first stage is essential as the performance drops significantly on all datasets. We hypothesize that contrastive pre-training on the intent datasets without using labels benefits the discrimination of semantically similar utterances. Additionally, the performance also drops if without supervised contrastive learning during the few-shot fine-tuning stage. Specifically, it drops by 2\%  on BANKING77 under the 5-shot setting; the reason is that BANKING77 is a single domain dataset with many similar intents, where supervised contrastive learning can explicitly discriminate semantically similar intents with very limited training examples. 
We also jointly train the first and second stages together, and compared with the proposed CPFT schema, we observe minimal improvements. The joint training is also costly as it requires retraining the model every time for new settings. 

\paragraph{Is contrastive pre-training beneficial to the target intent dataset? }
Additionally, we study whether contrastive pre-training can benefit the intent detection when excluding the target datasets. Specifically, we pre-train the model on the datasets except for the HWU64 dataset on the first stage and do few-shot learning on HWU64 during the second stage. Compared to the model without contrastive pre-training on the first stage, the performances are improved by 1.98\% and 1.21\% under 5-shot and 10-shot settings, respectively. The improvements indicate that the contrastive pre-training is helpful to transfer knowledge to new datasets. However, there are still performance drops compared to the contrastive pre-training, including the HWU64 dataset. Which shows that it is beneficial to include the target dataset during self-supervised contrastive learning. We leave whether self-supervised contrastive pre-training only on the target intent dataset benefits as a future study.

\paragraph{Is the training sensitive to hyper-parameters?}

We also study the effects of hyper-parameters of contrastive learning, \textit{i.e.}, the  temperature $\tau$ and weight $\lambda'$. We set $\tau \,{\in}\, \{0.05,0.1,0.3,0.5\}$ and $\lambda' \,{\in}\, \{0.01,0.03,0.05, 0.1\}$. In our primary experiments, we do not find $\tau$ has a notable influence during the self-supervised contrastive pre-training on the first stage.  Besides, we found that a batch size larger than 32 works well in the pre-training phase.
% as the model implicitly learn to discriminate semantically similar utterances without using labels. 
However, during the few-shot fine-tuning stage, when setting $\tau$ to a small value $0.05$, which heavily enforces the penalty to hard negative examples and $\lambda'$ to a large value $0.1$, which increases the weight of supervised contrastive learning loss, the performance drops significantly. In addition, the batch size  influences performance on this stage. Therefore, few-shot supervised contrastive loss is sensitive to hyper-parameters
% on the second stage performs more like a regularization loss 
when there are limited training examples. 
% We leave more studies to future work.

% Jianguo Zhang, Kazuma Hashimoto, Wenhao Liu, Chien-Sheng Wu, Yao Wan, S Yu Philip, Richard Socher, and Caiming Xiong. 2020. Discriminative nearest neighbor few-shot intent detection by transferring natural language inference. In Proceed- ings of the 2020 Conference on Empirical Methods in Natural Language Processing (EMNLP), pages 5064–5082.

% Shikib Mehri, Mihail Eric, and Dilek Hakkani-Tur. 2020b. Example-driven intent prediction with observers. arXiv preprint arXiv:2010.08684.

% Congying Xia, Chenwei Zhang, Hoang Nguyen, Jiawei Zhang, and Philip Yu. 2020. Cg-bert: Conditional text generation with bert for generalized few-shot in- tent detection. arXiv preprint arXiv:2004.01881.

% Baolin Peng, Chenguang Zhu, Michael Zeng, and Jianfeng Gao. 2020. Data augmentation for spoken language understanding via pretrained language models. arXiv preprint arXiv:2004.13952.

% Diederik P Kingma and Max Welling. 2013. Auto-encoding variational bayes. arXiv preprint arXiv:1312.6114.

% Alec Radford, Jong Wook Kim, Chris Hallacy, Aditya Ramesh, Gabriel Goh, Sandhini Agarwal, Girish Sastry, Amanda Askell, Pamela Mishkin, Jack Clark, et al. 2021. Learning transferable visual models from natural language supervision. Image, 2:T2.

% Inigo Casanueva, Tadas Temcinas, Daniela Gerz, Matthew Henderson, and Ivan Vulic. 2020. Efficient intent detection with dual sentence encoders. ACL 2020, page 38.

% Shikib Mehri, Mihail Eric, and Dilek Hakkani-Tur. 2020a. Dialoglue: A natural language understanding benchmark for task-oriented dialogue. preprint arXiv:2009.13570.

% Stefan Larson, Anish Mahendran, Joseph J. Peper, Christopher Clarke, Andrew Lee, Parker Hill, Jonathan K. Kummerfeld, Kevin Leach, Michael A. Laurenzano, Lingjia Tang, and Jason Mars. 2019. An Evaluation Dataset for Intent Classification and Out-of-Scope Prediction. In EMNLP, pages 1311– 1316.


\author{
  \textbf{Jianguo Zhang}$^1$~~~~ \textbf{Stephen Roller}$^2$~~~~  \textbf{Moya Chen}$^2$~~~~ \textbf{Paul Crook}$^2$~~~~ \\ \textbf{Zhiwei Liu}$^1$ \textbf{Yao Wan}$^3$~~~~ \textbf{Kun Qian}$^3$~~~~ \textbf{Philip S. Yu}$^1$  
  $^1$University of Illinois at Chicago, $^3$Huazhong University of Science and Technology\\ \\
 $^2$Facebook AI Research\\
%   { \textttt{jzhan51@uic.edu}}
{\texttt{\{jzhan51,zliu213,psyu\}@uic.edu}}
   { \texttt{\{mpchen,roller,pacrook\}@uic.edu}, \texttt{wanyao@hust.edu.cn} } \\
%   { \texttt{kazumah@google.com}, \texttt{cxiong@salesforce.com}} 
}
% \author{
%   \textbf{Jianguo Zhang}*~~~~ \textbf{Stephen Roller}†~~~~  \textbf{Moya Chen}†~~~~ \textbf{Paul Crook}†~~~~ \\ \textbf{Kun Qian}‡~~~~ \textbf{Zhiwei Liu}*~~~~ \textbf{Yao Wan}§~~~~ \textbf{Hu Xu}§~~~~ \textbf{Philip S. Yu}* \\
%   *University of Illinois at Chicago, §Huazhong University of Science and Technology\\ 
%  †Facebook AI Research\\
%  {\texttt{jzhan51@uic.edu}, \texttt{roller@fb.com}}
% % {\texttt{\{jzhan51,zliu213,psyu\}@uic.edu}}
% %   { \texttt{\{roller,mpchen,pacrook\}@fb.com}, \texttt{wanyao@hust.edu.cn} } \\
% %   { \texttt{kazumah@google.com}, \texttt{cxiong@salesforce.com}} 
% % 
% }
